Uncertainty-guided Source-free Domain Adaptation

Source-free domain adaptation (SFDA) aims to adapt a classifier to an unlabelled target data set by only using a pre-trained source model. However, the absence of the source data and the domain shift makes the predictions on the target data unreliable. We propose quantifying the uncertainty in the source model predictions and utilizing it to guide the target adaptation. For this, we construct a probabilistic source model by incorporating priors on the network parameters inducing a distribution over the model predictions. Uncertainties are estimated by employing a Laplace approximation and incorporated to identify target data points that do not lie in the source manifold and to down-weight them when maximizing the mutual information on the target data. Unlike recent works, our probabilistic treatment is computationally lightweight, decouples source training and target adaptation, and requires no specialized source training or changes of the model architecture. We show the advantages of uncertainty-guided SFDA over traditional SFDA in the closed-set and open-set settings and provide empirical evidence that our approach is more robust to strong domain shifts even without tuning.

==> figs/toy/CIFAR9_STL9_displot_entropy.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={CIFAR9->STL9},
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Entropy},
xmin=-0.383705954463738, xmax=2.47914948680024,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Density},
ymin=0, ymax=1.08320150186608,
ytick style={color=black}
]
\addplot [thick, green!50!black]
table {%
-0.253576161679012 0.0003953731252097
-0.240497790544869 0.000655412075324442
-0.227419419410725 0.00106457344506407
-0.214341048276582 0.00169454080363767
-0.201262677142439 0.00264368885011499
-0.188184306008295 0.00404318110742333
-0.175105934874152 0.0060627521259862
-0.162027563740008 0.00891531454772067
-0.148949192605865 0.012859327945928
-0.135870821471722 0.0181977616401986
-0.122792450337578 0.0252725386829076
-0.109714079203435 0.0344536122220006
-0.0966357080692917 0.0461223194547022
-0.0835573369351484 0.0606493600705268
-0.070478965801005 0.0783685813336239
-0.0574005946668616 0.0995485975618522
-0.0443222235327183 0.124364971732052
-0.031243852398575 0.15287608151113
-0.0181654812644316 0.185005754197919
-0.00508711013028823 0.22053522616897
0.00799126100385511 0.259105996426659
0.0210696321379985 0.300233832044695
0.0341480032721418 0.343332755154371
0.0472263744062852 0.387746543682571
0.0603047455404285 0.432784343044167
0.0733831166745719 0.477756577797823
0.0864614878087152 0.52200753108558
0.0995398589428586 0.564941669896598
0.112618230077002 0.606041881198048
0.125696601211145 0.64487903389502
0.138774972345289 0.681113472142799
0.151853343479432 0.714489993258809
0.164931714613575 0.744828454796953
0.178010085747719 0.772012355447407
0.191088456881862 0.795977575602062
0.204166828016005 0.816703021165068
0.217245199150149 0.834204282050122
0.230323570284292 0.848530689161744
0.243401941418436 0.859765419821725
0.256480312552579 0.868027648339567
0.269558683686722 0.873475253291512
0.282637054820866 0.876306360599149
0.295715425955009 0.876758088255386
0.308793797089152 0.875101289730673
0.321872168223296 0.87163082953605
0.334950539357439 0.866651851681886
0.348028910491582 0.860463440624904
0.361107281625726 0.85334181487664
0.374185652759869 0.84552554624597
0.387264023894012 0.837205147015701
0.400342395028156 0.828518710059352
0.413420766162299 0.819554242530266
0.426499137296442 0.810358120801604
0.439577508430586 0.800947978107991
0.452655879564729 0.791327562928474
0.465734250698873 0.78150084140243
0.478812621833016 0.771482907515351
0.491890992967159 0.761306030385214
0.504969364101303 0.751020226818037
0.518047735235446 0.740688863560498
0.531126106369589 0.730380734579062
0.544204477503733 0.720160645532836
0.557282848637876 0.710080679339366
0.570361219772019 0.700174020583209
0.583439590906163 0.690452576354371
0.596517962040306 0.680908799285196
0.609596333174449 0.671521269549786
0.622674704308593 0.662262886949346
0.635753075442736 0.653110079894737
0.64883144657688 0.644051313599255
0.661909817711023 0.635093370483836
0.674988188845166 0.626264322307823
0.68806655997931 0.617612718821094
0.701144931113453 0.609203168272844
0.714223302247596 0.60110907172986
0.72730167338174 0.593403707701901
0.740380044515883 0.586151089448778
0.753458415650026 0.579398013569386
0.76653678678417 0.573168498326205
0.779615157918313 0.567461416099941
0.792693529052456 0.562251620703873
0.8057719001866 0.557494334453523
0.818850271320743 0.553132072632993
0.831928642454886 0.549103017664562
0.84500701358903 0.545349566877095
0.858085384723173 0.541825793354094
0.871163755857316 0.538502772031652
0.88424212699146 0.535371091873024
0.897320498125603 0.532440330922894
0.910398869259747 0.529735731390079
0.92347724039389 0.527292696501239
0.936555611528033 0.525149979379977
0.949633982662177 0.523342518399671
0.96271235379632 0.521894801393483
0.975790724930463 0.520815452024994
0.988869096064607 0.520093483083848
1.00194746719875 0.519696412601108
1.01502583833289 0.519570234593593
1.02810420946704 0.51964109816807
1.04118258060118 0.519818472413429
1.05426095173532 0.519999536958701
1.06733932286947 0.520074509642854
1.08041769400361 0.519932580547136
1.09349606513775 0.519468059554102
1.1065744362719 0.51858627657061
1.11965280740604 0.517208729180343
1.13273117854018 0.515276986234325
1.14580954967433 0.512754953408431
1.15888792080847 0.509629292851839
1.17196629194261 0.505908041339185
1.18504466307676 0.50161774230946
1.1981230342109 0.496799634772873
1.21120140534504 0.491505566359953
1.22427977647919 0.485794279119004
1.23735814761333 0.47972854980781
1.25043651874747 0.473373385915616
1.26351488988162 0.466795152813365
1.27659326101576 0.460061221768887
1.2896716321499 0.453239562669564
1.30275000328405 0.44639770970582
1.31582837441819 0.43960070829056
1.32890674555233 0.432907963326475
1.34198511668648 0.426369270039966
1.35506348782062 0.420020619883429
1.36814185895476 0.413880547713772
1.38122023008891 0.407947771531259
1.39429860122305 0.402200673214228
1.40737697235719 0.396598830295899
1.42045534349134 0.391086423520093
1.43353371462548 0.385597011358512
1.44661208575962 0.380058960799939
1.45969045689377 0.374400792331914
1.47276882802791 0.368555824830442
1.48584719916205 0.362465738641022
1.4989255702962 0.356082935107332
1.51200394143034 0.349371784034968
1.52508231256448 0.342308969316501
1.53816068369863 0.33488315833121
1.55123905483277 0.327094160955894
1.56431742596691 0.31895165970957
1.57739579710106 0.310473535442137
1.5904741682352 0.301683815991989
1.60355253936934 0.292610341115861
1.61663091050349 0.283282339008962
1.62970928163763 0.273728203424923
1.64278765277177 0.263973801260636
1.65586602390592 0.25404160070625
1.66894439504006 0.243950788539531
1.6820227661742 0.233718367459578
1.69510113730835 0.223361033891032
1.70817950844249 0.2128974805531
1.72125787957663 0.202350683130354
1.73433625071078 0.19174973380293
1.74741462184492 0.18113087121386
1.76049299297906 0.17053750351366
1.77357136411321 0.160019195220636
1.78664973524735 0.1496297555715
1.79972810638149 0.13942469788424
1.81280647751564 0.129458418597226
1.82588484864978 0.119781464595965
1.83896321978392 0.110438221409428
1.85204159091807 0.101465273380716
1.86511996205221 0.0928905753890532
1.87819833318635 0.0847334522258548
1.8912767043205 0.0770053250834471
1.90435507545464 0.0697109720488251
1.91743344658878 0.062850074290697
1.93051181772293 0.0564187887725487
1.94359018885707 0.0504111209321648
1.95666855999122 0.044819937952925
1.96974693112536 0.039637549810334
1.9828253022595 0.0348558729823841
1.99590367339364 0.0304662634508307
2.00898204452779 0.0264591492413736
2.02206041566193 0.0228236035416896
2.03513878679608 0.0195469805487407
2.04821715793022 0.016614696993416
2.06129552906436 0.0140101952278471
2.07437390019851 0.011715080829019
2.08745227133265 0.00970939745872696
2.10053064246679 0.00797198785266565
2.11360901360093 0.00648089102464685
2.12668738473508 0.00521373730237478
2.13976575586922 0.0041481184794668
2.15284412700337 0.00326192460553014
2.16592249813751 0.0025336481764898
2.17900086927165 0.00194265966054195
2.1920792404058 0.00146945648087722
2.20515761153994 0.00109588312455912
2.21823598267408 0.000805315552067253
2.23131435380823 0.000582800547646142
2.24439272494237 0.000415141037531937
2.25747109607651 0.000290921590047752
2.27054946721066 0.0002004733705956
2.2836278383448 0.000135783450707542
2.29670620947894 9.03583055951339e-05
2.30978458061309 5.90546746881173e-05
2.32286295174723 3.78922943016802e-05
2.33594132288137 2.3862409256005e-05
2.34901969401552 1.47438537286801e-05
};
\addlegendentry{correct}
\addplot [thick, blue]
table {%
-0.168737109852771 6.91958965333167e-05
-0.156201782695459 0.000109485120775985
-0.143666455538146 0.000169757341202457
-0.131131128380833 0.000257964573808837
-0.118595801223521 0.000384254259021305
-0.106060474066208 0.000561157613011964
-0.0935251469088952 0.000803622683021782
-0.0809898197515825 0.0011288324576136
-0.0684544925942698 0.00155576140564837
-0.0559191654369571 0.00210445035912039
-0.0433838382796444 0.00279501856427785
-0.0308485111223317 0.00364647826731165
-0.018313183965019 0.00467546308704593
-0.00577785680770626 0.00589501596664027
0.00675747034960644 0.00731359489366916
0.0192927975069191 0.00893443700808354
0.0318281246642318 0.010755372405073
0.0443634518215446 0.0127691042165677
0.0568987789788573 0.0149638859245977
0.06943410613617 0.0173244505267203
0.0819694332934827 0.0198330002452019
0.0945047604507954 0.0224700658973269
0.107040087608108 0.0252150970348074
0.119575414765421 0.0280467387998949
0.132110741922734 0.0309428671321462
0.144646069080046 0.0338805600220781
0.157181396237359 0.0368362479771541
0.169716723394672 0.0397862891803457
0.182252050551984 0.0427081469143101
0.194787377709297 0.0455822200203657
0.20732270486661 0.0483942187771754
0.219858032023922 0.0511378248244446
0.232393359181235 0.053817260081233
0.244928686338548 0.0564493415626402
0.257464013495861 0.0590646262949839
0.269999340653173 0.0617073459649185
0.282534667810486 0.0644339740464967
0.295069994967799 0.0673104319377571
0.307605322125111 0.0704080989059266
0.320140649282424 0.0737989235407679
0.332675976439737 0.0775500308525374
0.34521130359705 0.0817182759593102
0.357746630754362 0.0863452143036824
0.370281957911675 0.0914529428672466
0.382817285068988 0.0970412193071695
0.3953526122263 0.103086187041005
0.407887939383613 0.109540924096545
0.420423266540926 0.116337893463612
0.432958593698239 0.123393207824565
0.445493920855551 0.130612442284498
0.458029248012864 0.137897551281736
0.470564575170177 0.145154291464245
0.483099902327489 0.152299445031137
0.495635229484802 0.15926710129285
0.508170556642115 0.1660133063409
0.520705883799427 0.172518540110631
0.53324121095674 0.17878772080329
0.545776538114053 0.184847745656923
0.558311865271366 0.190742914766222
0.570847192428678 0.196528898734951
0.583382519585991 0.202266144278879
0.595917846743304 0.208013713280152
0.608453173900616 0.213824486636172
0.620988501057929 0.219742428662227
0.633523828215242 0.22580222842351
0.646059155372555 0.232031171686156
0.658594482529867 0.238452636469098
0.67112980968718 0.245090241576949
0.683665136844493 0.25197149655354
0.696200464001805 0.259129859133452
0.708735791159118 0.266604412696245
0.721271118316431 0.27443688824754
0.733806445473743 0.282666380077445
0.746341772631056 0.291322714202803
0.758877099788369 0.300419887485953
0.771412426945682 0.30995118693871
0.783947754102994 0.319887455488922
0.796483081260307 0.330179492281919
0.80901840841762 0.340764835277597
0.821553735574932 0.351578306680899
0.834089062732245 0.362564879664494
0.846624389889558 0.373692821403303
0.859159717046871 0.384964819704862
0.871695044204183 0.396424977362947
0.884230371361496 0.408160142532606
0.896765698518809 0.420294932341355
0.909301025676121 0.432980832952816
0.921836352833434 0.446380725339875
0.934371679990747 0.460650908734164
0.946907007148059 0.475923043512891
0.959442334305372 0.492288363596852
0.971977661462685 0.509786055284768
0.984512988619997 0.528396979703477
0.99704831577731 0.548043088458621
1.00958364293462 0.568592109749488
1.02211897009194 0.589866495317243
1.03465429724925 0.611655288696382
1.04718962440656 0.633727507130806
1.05972495156387 0.655845770866201
1.07226027872119 0.67777917776432
1.0847956058785 0.699314715843466
1.09733093303581 0.720266758539253
1.10986626019312 0.740484359890826
1.12240158735044 0.759856161247399
1.13493691450775 0.778312769931095
1.14747224166506 0.795826520342694
1.16000756882238 0.812408621233101
1.17254289597969 0.828103850336279
1.185078223137 0.842983170561927
1.19761355029431 0.8571348727963
1.21014887745163 0.87065504261677
1.22268420460894 0.883638243679476
1.23521953176625 0.896169268350584
1.24775485892356 0.908316618522022
1.26029018608088 0.920128078725939
1.27282551323819 0.931628397041315
1.2853608403955 0.942818782741732
1.29789616755282 0.953677742886262
1.31043149471013 0.964162761139518
1.32296682186744 0.974212469182186
1.33550214902475 0.983749218488501
1.34803747618207 0.992682231822618
1.36057280333938 1.00091169085557
1.37310813049669 1.00833411265003
1.385643457654 1.01484915080656
1.39817878481132 1.02036756423719
1.41071411196863 1.02481963027925
1.42324943912594 1.02816288000936
1.43578476628326 1.03038784002594
1.44832009344057 1.03152056786029
1.46085542059788 1.03162118005596
1.47339074775519 1.03077821714979
1.48592607491251 1.02909942174911
1.49846140206982 1.02670014700665
1.51099672922713 1.02369100482581
1.52353205638444 1.02016641293164
1.53606738354176 1.01619540597863
1.54860271069907 1.01181552741766
1.56113803785638 1.00702996833533
1.57367336501369 1.00180753699242
1.58620869217101 0.996084667223003
1.59874401932832 0.989768575761686
1.61127934648563 0.982740845272895
1.62381467364295 0.974861055940057
1.63635000080026 0.96597048651178
1.64888532795757 0.955896226448326
1.66142065511488 0.94445619004051
1.6739559822722 0.931465464997601
1.68649130942951 0.916744188268251
1.69902663658682 0.900126795607595
1.71156196374413 0.881472136381245
1.72409729090145 0.860673672915191
1.73663261805876 0.837668855842521
1.74916794521607 0.812446801738364
1.76170327237339 0.785053572501713
1.7742385995307 0.755594612541081
1.78677392668801 0.724234174002593
1.79930925384532 0.691191795966365
1.81184458100264 0.656736070087706
1.82437990815995 0.621176023415203
1.83691523531726 0.58485050624735
1.84945056247457 0.548116027990336
1.86198588963189 0.511333569488158
1.8745212167892 0.474855025858288
1.88705654394651 0.439010078699451
1.89959187110383 0.404094413523187
1.91212719826114 0.370360228889759
1.92466252541845 0.33800987902284
1.93719785257576 0.307193231834092
1.94973317973308 0.278008930027254
1.96226850689039 0.250509274305092
1.9748038340477 0.224707990342143
1.98733916120501 0.200589784583145
1.99987448836233 0.178120408282633
2.01240981551964 0.157255968147806
2.02494514267695 0.137950435749981
2.03748046983426 0.120160668206046
2.05001579699158 0.103848686421777
2.06255112414889 0.0889813846656246
2.0750864513062 0.0755281969847412
2.08762177846352 0.0634574749226334
2.10015710562083 0.0527324176146038
2.11269243277814 0.0433073463234163
2.12522775993545 0.0351249578784351
2.13776308709277 0.0281149645726052
2.15029841425008 0.0221942750921761
2.16283374140739 0.0172686321521757
2.1753690685647 0.0132354295549689
2.18790439572202 0.00998730481885376
2.20043972287933 0.00741605118092867
2.21297505003664 0.0054164105772512
2.22551037719396 0.00388938338790777
2.23804570435127 0.00274480132549698
2.25058103150858 0.00190303467381376
2.26311635866589 0.00129582369105363
2.27565168582321 0.000866320699461838
2.28818701298052 0.000568495034660351
2.30072234013783 0.000366085245908616
2.31325766729514 0.000231285082614239
2.32579299445246 0.000143329077890276
};
\addlegendentry{incorrect}
\end{axis}

\end{tikzpicture}

